Crystallization of an exciton superfluid

Indirect excitons -- pairs of electrons and holes spatially separated in semiconductor bilayers or quantum wells -- are known to undergo Bose-Einstein condensation and to form a quantum fluid. Here we show that this superfluid may crystallize upon compression. However, further compression results in quantum melting back to a superfluid. This unusual behavior is explained by the effective interaction potential between indirect excitons which strongly deviates from a dipole potential at small distances due to many-particle and quantum effects. Based on first principle path integral Monte Carlo simulations, we compute the complete phase diagram of this system and predict the relevant parameters necessary to experimentally observe exciton crystallization in semiconductor quantum wells.

==> add_text.tex <==
%\documentclass[a4paper,10pt]{article}
%\usepackage[utf8x]{inputenc}
%\usepackage{graphicx}

%\begin{document}

{\Large \bf Supplementary Material to the article \\[1ex]
``Crystallization of an exciton superfluid''}\\[1ex]
J. B\"oning, A. Filinov, and M. Bonitz \\[2ex]

\noindent
Here we present details of our computations of the phase diagram of indirect excitons in two supplementary figures.
Figure \ref{figs1} illustrates the computation  of the winding number versus temperature (left) and the finite size scaling for the critical temperature of the BKT transition (right). The scaling allows us to extrapolate to an infinite system, $L\rightarrow \infty$ and thus make predictions for a macroscopic system.

\begin{figure}[ht]
\begin{center}
\includegraphics[width=1.0 \textwidth]{fig_s1} 
\end{center}
\vspace{-0.2cm}
\caption{(a) Temperature dependence of the winding number $\langle W^2 \rangle(T)$ for two exciton numbers $N=56$ and $170$ at a density of $n a^{*2}_B=5 \cdot 10^{-3}$. The Berezinskii-Kosterlitz-Thouless transition temperature $T_c(N)$ is determined by the condition~\cite{nelson_universal_1977}, $\langle W^2 \rangle(T_c(N))=4/\pi$, shown by the horizontal dashed line. One observes a systematic shift of $T_c(N)$ to lower values with the increase of the system size $N$. (b) System size dependence of $T_c(L=\sqrt{N/n})$ for three densities: $n a^{*2}_B=5 \cdot 10^{-3}, 10^{-2}, 2\cdot 10^{-2} $. The extrapolation to the thermodynamic limit, $T_c(L\rightarrow \infty)$, is obtained by fitting the simulation data by the equation: $T_c(L)=T_c(\infty)+ b/\ln^2(L)$ . It is a direct consequence of the Kosterlitz-Thouless renormalization group analysis \cite{nelson_universal_1977} which is considered to be exact in the asymptotic regime of large $L$.}
\label{figs1}
\end{figure}

\newpage
The second figure explores the nature of the melting transition at constant density. We analyze the number of defects, i.e. the number of particles (the probability) not having six nearest neighbors. There is a sharp increase of the number of defects at the melting point which is in disagreement with the KTNHY scenario.
A possible alternative to the KTNHY thery of melting in 2D is a first order solid-liquid phase transition, with an exponential decay of $g_6(r)$. This is
not observed in our simulations, possibly due to a limited system size. In the simulations, we observe an accumulation of the defects at grain boundaries formed between small crystallites. This, as was recently verified for classical 2D systems, forces the phase transition to be of first order~\cite{Hart}. To answer this question for the present system would require extensive additional simulations.

\begin{figure}[h]
\begin{center}
\includegraphics[width=0.85 \textwidth]{fig_s2} 
\end{center}
\vspace{-0.2cm}
\caption{Temperature dependence of the defect fraction at density $n a^{*2}_B=2.2 \cdot 10^{-3}$ and particle numbers $N=501-505$ (vertically aligned dots), which characterizes the ordered and disordered phases. A Voronoi analysis was performed  to provide access to local distortions of the hexagonal symmetry which are characterized by $1-P_6$ where $P_6$ is the probability that a particle has $6$ nearest neighbors. The defect fraction shows a sharp jump at 
$T \sim 10^{-3}$Ha$^*$. This is in disagreement with the KTNHY theory, which predicts a continuous unbinding of dislocations in the hexatic phase indicated by a continuous variation of the critical exponent  $\eta_6(T) \leq 1/4$
and the bond angular correlation function $g_6(r)\sim r^{-\eta_6(T)}$. In contrast,
we observe an abrupt transition to quasi-long-range angular order with $\eta_6(T)\sim 2$, cf. Fig.~2. of the main article.} 
\label{figs2}
\end{figure}


\begin{thebibliography}{24}
\bibitem{nelson_universal_1977} D.~R. Nelson and J.~M.Kosterlitz, Phys. Rev. Lett. {\bf 39}, 1201 (1977)
\bibitem{Hart} P.~Hartmann et. al., Phys. Rev. Lett. {\bf 105}, 115004 (2010)
\end{thebibliography}


%\end{document}

